Self-supervised Co-training for Video Representation Learning

The objective of this paper is visual-only self-supervised video representation learning. We make the following contributions: (i) we investigate the benefit of adding semantic-class positives to instance-based Info Noise Contrastive Estimation (InfoNCE) training, showing that this form of supervised contrastive learning leads to a clear improvement in performance; (ii) we propose a novel self-supervised co-training scheme to improve the popular infoNCE loss, exploiting the complementary information from different views, RGB streams and optical flow, of the same data source by using one view to obtain positive class samples for the other; (iii) we thoroughly evaluate the quality of the learnt representation on two different downstream tasks: action recognition and video retrieval. In both cases, the proposed approach demonstrates state-of-the-art or comparable performance with other self-supervised approaches, whilst being significantly more efficient to train, i.e. requiring far less training data to achieve similar performance.

==> sec/discussion.tex <==
\section{Discussion}

\paragraph{Comparison to CMC.}
{\bf (1)~Difference.}
The training scheme of CMC~\cite{Tian19} is fundamentally different to that of CoCLR.
CMC aims to maximize the mutual information between multiple domains of the same video clip, 
{\em i.e.}~learning the correspondence between its RGB and Flow representations.
Thus, the proxy task defined by CMC is still limited to be {\em instance discrimination}.
However, CoCLR goes beyond this by explicitly allowing \textbf{multiple instances from the same domain} to be positive pairs, 
specifically, the most similar clip to one query sample based on flow representation is treated as a positive pair in the RGB domain,
this design allows to exploit the complementary nature between different modalities,
in addition, we also adopts a noise-tolerant MIL-NCE loss.
{\bf (2)~Experiments.}
We carry out a comparison on UCF101, 
by training a CMC model with the same backbone~(S3D) as ours for the same number of epochs~(fair comparison with CoCLR). Specifically, two networks for both RGB and Flow streams are trained simultaneously by maximizing the mutual information among three views $\texttt{RGB}_t, \texttt{RGB}_{t+k}, \texttt{Flow}_t$, as in CMC section 4.2.
We evaluated the RGB model by linear probing:
the CMC model gets 55.2\% on UCF101~(note that, 
the model in original CMC paper actually finetunes the entire network, and only get 59.1\%, 
this is significantly lower than all of our finetune models in Table~1, above $78\%$),
whereas the CoCLR-RGB model gets 70.2\% by linear probing.



==> sec/save.tex <==
\section*{Figure and Table}

\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}

\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}


==> sup/python_support.tex <==
% Default fixed font does not support bold face
\DeclareFixedFont{\ttb}{T1}{txtt}{bx}{n}{6} % for bold
\DeclareFixedFont{\ttm}{T1}{txtt}{m}{n}{6}  % for normal

% Custom colors
\definecolor{deepblue}{rgb}{0,0,0.5}
\definecolor{deepred}{rgb}{0.6,0,0}
\definecolor{deepgreen}{rgb}{0,0.5,0}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}


\definecolor{codeblue}{rgb}{0.25,0.5,0.5}
\lstset{
	backgroundcolor=\color{white},
	basicstyle=\fontsize{8.2pt}{8.2pt}\ttfamily\selectfont,
	columns=fullflexible,
	breaklines=true,
	captionpos=b,
	commentstyle=\color{codeblue},
	keywordstyle=\color{codegreen},
	stringstyle=\color{codepurple}
	%  frame=tb,
}

%\lstdefinestyle{mystyle}{
%	%backgroundcolor=\color{backcolour},   
%	commentstyle=\color{codegreen},
%	keywordstyle=\color{magenta},
%	numberstyle=\tiny\color{codegray},
%	stringstyle=\color{codepurple},
%	basicstyle=\ttfamily\scriptsize,
%	breakatwhitespace=false,         
%	breaklines=true,                 
%	captionpos=b,                    
%	keepspaces=true,                 
%	%numbers=left,                    
%	numbersep=5pt,                  
%	showspaces=false,                
%	showstringspaces=false,
%	showtabs=false,                  
%	tabsize=2
%}
%
%\lstset{style=mystyle}



==> sup/source.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table}[!htb]
\footnotesize
	\centering
		\begin{tabu}{l|lcc} \hline
		Method & Dataset (duration) & Arch. & Depth \\ \hline
		CBT       & K600+ (273d)      & S3D & $2+   =23$   \\
		MIL-NCE   & HTM (15y)         & S3D & 23      \\
		MIL-NCE   & HTM (15y)         & I3D & 22      \\
		XDC  	  & IG65M~(21y)      & R(2+1)D18 & 26   \\ % R(2+1)D18
		ELO       & Youtube8M- (8y)       & R(2+1)D50 & 65  \\ % R(2+1)D50
		\hline
		OPN          & UCF (1d)         & VGG16 & 14    \\ % VGG16
		3D-RotNet    & K400 (28d)       & R3D18 & 17     \\ % R3D18
		ST-Puzzle      & K400 (28d)       & R3D18 & 17    \\ % R3D18
		VCOP        & UCF (1d)        & R(2+1)D18 & 26  \\ % R(2+1)D18
		DPC           & K400 (28d)      & 2D3D-R34 & 33   \\ % R-2D3D-34
		CBT           & K600+ (273d)    & S3D & 23      \\
		DynamoNet  & Youtube8M-1 (1.9y)       & STCNet101 & 133  \\ % STCNet-101
		SpeedNet  & K400 (28d)       & S3D-G & 23       \\
		AVTS     & K400 (28d)       & I3D & 22       \\
		AVTS     & AudioSet (240d)       & MC3 & 17       \\
		XDC      & IG65M~(21y)       & R(2+1)D18 & 26    \\ % R(2+1)D18
		GDT         & K400 (28d)       & R(2+1)D18 & 26     \\ %R(2+1)D18
		MIL-NCE        & HTM (15y)        & S3D  & 23      \\
		ELO  & Youtube8M-2 (13y)        & R(2+1)D50 & 65       \\ %R(2+1)D50
		\hline
		\textbf{CoCLR}          & UCF (1d)    & S3D & 23 \\
		\textbf{CoCLR}          & K400 (28d)  & S3D & 23 \\
		\hline
		\end{tabu}
	\vspace{5pt}
	\caption{Comparison with state-of-the-art approaches.
		In the left columns, we show the pre-training setting, \eg~dataset, resolution, architectures with encoder depth, modality.
		In the right columns, the top-1 accuracy is reported on the downstream action classification task for different datasets, 
		\eg~UCF, HMDB, K400.
		The dataset parenthesis shows the total video duration in time (\textbf{d} for day, \textbf{y} for year).
		`Frozen \xmark' means the network is end-to-end finetuned from the pretrained representation, 
		  shown in the top half of the table;
		`Frozen \cmark' means the pretrained representation is fixed and classified with a linear layer, 
		  shown in the bottom half.
		For input, {\color{blue}`V' refers to visual only~(colored with blue)}, `A' is audio, `T' is text narration.
		CoCLR models with $\dagger$ refer to the two-stream networks, 
		where the predictions from RGB and Flow networks are averaged.
		}\vspace{-5mm}
	
	\label{table:sota-classification}
\end{table}




==> table/ct_analysis.tex <==
\begin{table}[h!]
\footnotesize
	\caption{Effectiveness of Co-training: video NN-retrieval within UCF training set.}
	\label{table:ct-effectiveness}
	\centering
	\begin{tabular}{ll|lll|lll}
	\hline
	Method                       & Input & R@1  & P@1  & Overlap@1            & R@5  & P@5  & Overlap@5            \\ \hline
	\multirow{2}{*}{CT}        & RGB   & -    & -    & \multirow{2}{*}{-}   & -    & -    & \multirow{2}{*}{-}   \\
	                           & Flow  & -    & -    &                      & -    & -    &                      \\ \hline
	\multirow{2}{*}{w/o CT}    & RGB   & 30.9 & 30.9 & \multirow{2}{*}{2.3} & 47.8 & 27.0 & \multirow{2}{*}{4.5} \\
	                           & Flow  & 40.1 & 40.1 &                      & 64.0 & 35.1 &                      \\ \hline
	
	\end{tabular}
\end{table}


==> table/ct_classification.tex <==
\begin{table}[h!]
\footnotesize
	\caption{Ablation: effectiveness of Co-training on UCF action classification.}
	\label{table:ct-classification}
	\centering
	\begin{tabular}{ll|ll}
		\hline 
	Method      & Input & UCF-linear probe & UCF-finetune \\ \hline
	Co-Training & RGB   & \textbf{67.5}   & \textbf{81.4}\\ \hline
	NCE         & RGB   & 46.2            & 74.4       \\
	NCE         & Flow  & 64.9            & ?          \\ \hline
	\end{tabular}
\end{table}

==> table/ct_frequency.tex <==
\begin{table}[h!]
\footnotesize
	\caption{Frequency of bootstrap, experimented on UCF101 and evaluated by action classification.
	All Co-training methods are initialized the same way and trained for 250 epochs.
    The infinite frequency denotes both representations are optimized simultaneously.}
	\label{table:frequency}
	\centering
	\begin{tabular}{ll|ll}
		\hline 
	Method      & Bootstrap frequency     & UCF-linear probe & UCF-finetune \\ \hline
	Co-Training & $\infty$ (simultaneous) & 65.2            & 80.8          \\
	Co-Training & every 50 epochs         & ?               & ?             \\
	Co-Training & every 100 epochs        & 67.5            & 81.4          \\ \hline
	\end{tabular}
\end{table}

==> table/ct_k400.tex <==
\begin{table}[h!]
\footnotesize
	\caption{Scale-up Co-training method to K400 and its subset.
		Our Co-training method consistently shows effectiveness 
		comparing with the NCE baseline on different dataset sizes.
		The classification performance gets better when more data is used for self-supervised pre-training.}
	\label{table:ct-k400}
	\centering
		\begin{tabular}{lll|ll}
		\hline
		Method & Dataset & Input & UCF-linear probe & UCF-finetune \\ \hline
%		NCE             & K200-15 & RGB   & 48.5             & 80.0         \\
%		Co-training     & K200-15 & RGB   & 66.7             & 84.6*        \\ \hline
		NCE             & K400-30 & RGB   & 53.5             & -            \\
		Co-training     & K400-30 & RGB   & 73.8             & 84.4         \\ \hline
		NCE             & K400-50 & RGB   & -                & -            \\
		Co-training     & K400-50 & RGB   & 76.3      & 87.0  \\ \hline
		NCE             & K400 (100\%)    & RGB   & -                & -            \\
		Co-training     & K400 (100\%)    & RGB   & $\approx$80      & $\approx$90            \\ \hline
		\end{tabular}
\end{table}

==> table/more_ds.tex <==

\begin{table}[h!]
\footnotesize
	\centering
		\begin{tabular}{cc|ccc|ccc|ccc}
			\hline
			\multirow{2}{*}{Method} & \multirow{2}{*}{Date} & \multicolumn{3}{c|}{UCF}         & \multicolumn{3}{c|}{HMDB}   & \multicolumn{3}{c}{K400}          \\ \cline{3-11} 
			& & 5 shots & 10 shots & 20 shots   &  5 shots & 10 shots & 20 shots   &  5 shots & 10 shots & 20 shots   \\ \hline
			
		 DPC~\cite{Han19}       & ICCVW2019   & 31.8 & 41.0 & 58.2    & 18.3  & 24.0 & 33.0   & ??  & ??    & ?? \\ 
		 MIL-NCE~\cite{Miech20} & CVPR2020    & ??   & ??   & 67.7    & 21.1  & 25.2 & 39.9   & ??  & ??    & ?? \\ 
		\hline
		 CoCLR - UCF            & 2020        & 50.2 & 60.2 & 69.0    & 21.8  & 29.3 & 37.0   & ??  & ??    & ?? \\ 
		 % CoCLR~$\dagger$ - UCF  & 2020        & ??   & ??   & ??      & ??    & ??   & ??     & ??  & ??    & ?? \\ 
		 CoCLR- K400            & 2020        & 45.7 & 57.3 & 72.3    & 23.4  & 33.6 & 42.0   & -   & -     & ?? \\ 
		 % CoCLR~$\dagger$- K400  & 2020        & -    & -    & -       & -     & -    & -      & -   & -     & ?? \\ 
		    \hline
		\end{tabular}
		\vspace{5pt}
		\caption{Compare with others on Nearest-Neighbour video retrieval on UCF101 and HMDB51.
		Testing set video is used to retrieval training set videos and R@k is reported.
		If not specified, other methods are pre-trained on UCF101. 
		We also provide our method pre-trained on K400 for future research. 
	\TODO{need to check new papers}}
	\label{table:fewshot}
\end{table}


==> table/sota_retrieval_bp.tex <==
\setlength{\tabcolsep}{2pt}
\begin{table}[h!]
\footnotesize
	\centering
		\begin{tabular}{cc|cccc|cccc|cccc}
			\hline
			\multirow{2}{*}{Method} & \multirow{2}{*}{Date} & \multicolumn{4}{c|}{UCF}         & \multicolumn{4}{c|}{HMDB}   & \multicolumn{4}{c}{K400}          \\ \cline{3-14} 
			& & R@1 & R@5 & R@10 & R@20  & R@1 & R@5 & R@10 & R@20  & R@1 & R@5 & R@10 & R@20  \\ \hline
			
	         Jigsaw~\cite{Noroozi16} & 2016 & 19.7 & 28.5 & 33.5  & 40.0    & -    & -    & -    & -   & - & - & - & -   \\
		  OPN~\cite{Lee17} &     2017       & 19.9 & 28.7 & 34.0  & 40.6  & -    & -    & -     & -      & - &  - & - & - \\
		  Buchler~\cite{Buchler18}& 2018 & 25.7 & 36.2 & 42.2  & 49.2   & -    & -    & -     & -   & - & - & - & - \\
		 VCOP~\cite{Xu19vcop} & 2019  & 14.1 & 30.3 & 40.4  & 51.1    & 7.6  & 22.9 & 34.4  & 48.8   & - & -  & - & -  \\
		 %DPC~\cite{Han19} &  2019        & ?? & ?? & ??  & ??   & ?? & ?? & ??  & ??    & ?? & ?? & ?? & ?? \\ 
		 VCP~\cite{Luo20} &  2020      & 18.6 & 33.6 & 42.5  & 53.5   & 7.6  & 24.4 & 36.3  & 53.6   & - & -& -& - \\ 
		 %MIL-NCE~\cite{Miech20} & 2020  & 11.7* & 22.6* & 30.9*  & 42.6*   & ?? & ?? & ??  & ??    & ?? & ?? & ?? & ?? \\ 
		\hline
		  CoCLR-RGB & 2020      & 51.4 & 67.9 & 74.9  & 81.1   & 19.5  & 43.3  & 55.6  & 67.7    & ?? & ?? & ?? & ?? \\ 
		  CoCLR-Flow & 2020      & 51.4 & 67.9 & 74.9  & 81.1   & 19.5  & 43.3  & 55.6  & 67.7    & ?? & ?? & ?? & ?? \\ 
		 % CoCLR~$\dagger$- UCF  &2020     & -    & -    & -     & -     & -     & -    & -    & -        & ?? & ?? & ?? & ?? \\ 
		  %CoCLR- K400  & 2020     & -    & -    & -     & -      & 16.7* & 36.9* & 48.7* & 62.4*   & ?? & ?? & ?? & ?? \\ 
		  % CoCLR~$\dagger$- K400 & 2020      & -    & -    & -     & -     & -     & -    & -    & -        & ?? & ?? & ?? & ?? \\ 
		    \hline
		\end{tabular}
		\vspace{5pt}
		\caption{Compare with others on Nearest-Neighbour video retrieval on UCF101 and HMDB51.
		Testing set video is used to retrieval training set videos and R@k is reported.
		As for K400, 
		the $k$-NN retrieval is conducted on its validation set~(20k videos for 400 classes), 
		that is, using validation set videos to retrieve other validation set videos.
		The DPC and MIL-NCE models are taken from ~\cite{dpc_code, mil_nce_code}.
	\TODO{need to check new papers}}
	\label{table:retrieval}
\end{table}

0.1668 5NN acc = 0.3690 10NN acc = 0.4865 20NN acc = 0.6244
